Ill-posedness of degenerate dispersive equations

In this article we provide numerical and analytical evidence that some degenerate dispersive partial differential equations are ill-posed. Specifically we study the K(2,2) equation $u_t = (u^2)_{xxx} + (u^2)_{x}$ and the "degenerate Airy" equation $u_t = 2 u u_{xxx}$. For K(2,2) our results are computational in nature: we conduct a series of numerical simulations which demonstrate that data which is very small in $H^2$ can be of unit size at a fixed time which is independent of the data's size. For the degenerate Airy equation, our results are fully rigorous: we prove the existence of a compactly supported self-similar solution which, when combined with certain scaling invariances, implies ill-posedness (also in $H^2$).

==> ARXIV FILES/gsmacros.tex <==
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\paren}[1]{\left(#1\right)}
\newcommand{\bracket}[1]{\left[#1\right]}
\newcommand{\set}[1]{\left\{#1\right\}}

\newcommand{\bigo}{\mathrm{O}}
\newcommand{\matlab}{\textsc{Matlab} }
\newcommand{\mean}[1]{\left\langle#1\right\rangle}
\newcommand{\eps}{\epsilon}
\newcommand{\vareps}{\varepsilon}
\newcommand{\To}{\longrightarrow}
\newcommand{\dz}{\partial_{z} }
\newcommand{\dx}{\partial_{x} }
\newcommand{\ddx}{\frac{d}{dx}}
\newcommand{\ddr}{\frac{d}{dr}}
\newcommand{\sinc}{\mathrm{sinc}}
\newcommand{\even}{\mathrm{even}}
\newcommand{\cont}{\mathrm{cont.}}
\newcommand{\comp}{\mathrm{comp.}}
\newcommand{\cut}{{\mathrm{cut}}}
\newcommand{\ind}{{\mathrm{ind}}}
\newcommand{\rad}{{\mathrm{rad}}}
\newcommand{\embd}{{\mathrm{em}}}
\newcommand{\spn}{{\mathrm{span}}}
\newcommand{\rmax}{r_{\max}}
\newcommand{\xmax}{x_{\max}}
%\newcommand{\i}{\mathmr{i}}
\newcommand{\grad}{\nabla}

\newcommand{\ess}{\mathrm{ess}}
\newcommand{\kerg}{\ker_{\mathrm{g}}}
%\newcommand{\ker}{\mathrm{ker}}
\newcommand{\ran}{\mathrm{ran}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\kdv}{\mathrm{KdV}}
\newcommand{\dist}{\mathrm{d}}
\newcommand{\dom}{\mathrm{dom}}
\newcommand{\Rlam}{\partial_{\lambda} R}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\Rmin}{R_{\min}}


\newcommand{\lip}{\mathrm{lip.}}
\newcommand{\disc}{\mathrm{disc}}
\newcommand{\dzz}{\partial_{z}^{2}}
\newcommand{\zz}{{zz}}
\newcommand{\bXYZ}{{\bf XYZ}}
\newcommand{\h}[1]{{H^{#1}}}
\newcommand{\ha}{{H^1_a}}
\newcommand{\hinta}{{H^1 \cap H^1_a}}

\newcommand{\ltwo}{{L^2}}
\newcommand{\linf}{{L^\infty}}
\newcommand{\inner}[2]{\left\langle #1,#2\right\rangle}
\newcommand{\twodcolvec}[2]{\begin{pmatrix} #1\\ #2\end{pmatrix}}
%\newcommand{\twobytwo}[4]{\left(\begin{array}{cc} #1 & #2\\ #3 & #4\end{array}\right)}
\newcommand{\twobytwo}[4]{\begin{pmatrix} #1 & #2\\ #3 & #4\end{pmatrix}}
\newcommand{\threedcolvec}[3]{\begin{pmatrix} #1\\ #2\\#3\end{pmatrix}}
\newcommand{\threedrowvec}[3]{\left( #1,\quad #2,\quad#3\right)}
\newcommand{\hh}{{H^2}}
\newcommand{\dt}{\partial_{t}}
\newcommand{\dc}{\partial_{c}}
\newcommand{\dxi}{\partial_{\xi}}
\newcommand{\dtau}{\partial_{\tau}}
\newcommand{\dyy}{\partial_{yy}}
\newcommand{\dy}{\partial_{y}}
\newcommand{\f}{\phi}
\newcommand{\g}{\gamma}
\newcommand{\gt}{\dot{\gamma}}
\newcommand{\thetadot}{\dot{\theta}}
\newcommand{\co}{ {c_{0}}}
\newcommand{\ct}{{c(t)}}
\newcommand{\thetat}{{\theta(t)}}
\newcommand{\dcdt}{{\dot{c}}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\nn}{\nonumber}
\newcommand{\kap}{\kappa}
\newcommand{\lam}{\lambda}
\newcommand{\E}{\mathcal{E}}
\newcommand{\inv}{^{-1}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\N}{\mathcal{N}}
%\newcommand{\R}{\mathbb{R}}
%\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\calk}{\mathcal{K}}
\newcommand{\call}{\mathcal{L}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calf}{\mathcal{F}}
\newcommand{\caln}{\mathcal{N}}
\newcommand{\calh}{\mathcal{H}}
\newcommand{\Low}{\mathcal{L}}
\newcommand{\by}{\bold{y}}
\newcommand{\bz}{\bold{z}}
\newcommand{\bv}{\bold{v}}
\newcommand{\bF}{\bold{f}}
\newcommand{\sech}{\mathrm{sech}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\nb}{\noindent\textbf{N.B.}\quad}
%\newcommand{\qed}{\begin{flushright}{$\blacksquare$}\end{flushright}}
\newcommand{\local}{\mathrm{local}}
\newcommand{\exist}{\mathrm{exist}}
%\newcommand{\proof}{\noindent \textbf{Proof}:\quad}

\newtheorem{thm}{Theorem}
\newtheorem{prop}{Proposition}[section]
%\newtheorem{cor}[prop]{Corollary}
\newtheorem{lem}[prop]{Lemma}
\newtheorem{claim}[prop]{Claim}
\newtheorem{conj}[prop]{Conjecture}
\newtheorem{rem}[prop]{Remark}
\newtheorem{ex}{EXAMPLE}[section]
\newtheorem{example}[prop]{Example}
\newtheorem{exmple}[prop]{Example}
\newtheorem{defn}[prop]{Definition}
\newtheorem{definition}[prop]{Definition}
\newtheorem{assumption}[prop]{Assumption} 

